RAN-JEPA: An Action-Conditioned World Model for Energy-efficient Mobile Network Control

Operational mobile networks are rich in observations but poor in interventions: they continuously generate large volumes of passive telemetry, while controlled action--response trajectories remain comparatively scarce and costly to collect. This observation--intervention asymmetry is a central obstacle to building practical world models for RAN control. We address this problem with RAN-JEPA, an action-conditioned world model that separates representation learning from intervention learning. The model first learns a predictive latent representation from observation-only network data, adapts that representation to the target deployment domain, and then learns action-conditioned latent dynamics from controlled sleep/wake trajectories while keeping the encoder fixed. We evaluate RAN-JEPA using public operator performance data for pretraining and a real-equipment four-cell 5G testbed for domain adaptation, post-training, and control. Across four future 15-minute intervals, RAN-JEPA achieves lower action-conditioned prediction error than a GPT-2 world-model baseline and a mechanistic rule, while remaining close to a strong persistence reference. What-if evaluation further shows that the model produces distinct and coherent future trajectories under matched SLEEP and KEEP plans. In closed-loop control, RAN-JEPA consistently supports higher sleep ratios than the two baselines at comparable congestion cost. These results show that observation-first, action-conditioned learning can turn abundant passive telemetry and limited intervention data into a practical predictive model for energy-aware RAN control.

==> section/related_works.tex <==
\section{Why Action-Conditioned JEPA for Mobile Network Control?}
\label{sec:why_jepa}

The motivation for an action-conditioned JEPA world model follows from three observations. 
First, forecasting future network measurements is not equivalent to predicting network 
responses under alternative control actions. Second, the trajectories needed to learn such 
responses are much scarcer than ordinary telecom observations. Third, although several model 
families can exploit passive data, JEPA provides a particularly direct route for connecting 
predictive representation learning with subsequent action-conditioned latent dynamics.

\subsection{From Network Forecasting to Action-Conditioned World Modeling}
\label{subsec:forecasting_vs_action}

Modern communication networks generate rich multivariate time series, and increasingly capable 
forecasting models can learn regularities in traffic, KPIs, counters, channel measurements, and 
other operational signals. Such models are valuable for tasks including capacity prediction, 
anomaly anticipation, resource planning, and proactive maintenance. Their primary question, 
however, is observational: given the recent network history, what is likely to happen next?

Network control requires a different capability. A controller must compare alternative 
decisions that may intentionally move the system away from the trajectory that would otherwise 
occur. For example, when considering whether to place a cell or carrier into an energy-saving 
state, the relevant question is not only how traffic or throughput will evolve if the current 
configuration is maintained. The controller must estimate how those quantities would evolve 
\emph{under each candidate action}.

Simply adding configuration variables to the input of a conventional forecasting model does 
not by itself resolve this problem. Historical configuration values are generated by existing 
control policies, operational rules, and human decisions. They therefore reflect the action 
distribution present in historical data rather than systematic exploration of alternative 
actions. A predictor may achieve high accuracy on observed trajectories while remaining 
unreliable when queried with actions that are infrequent or absent in its training data.

An action-conditioned world model makes the role of control explicit. It represents network 
evolution as a function of both the current network state and a candidate action, enabling the 
same learned dynamics to be queried repeatedly under alternative configurations. This 
capability supports model-based control because an external planner or optimizer can perform 
candidate-action rollouts and compare their predicted consequences without binding the learned 
model to a single reward function. Recent work on mobile-network energy saving has demonstrated 
the feasibility of this approach using an explicitly action-conditioned world model 
\cite{bouton2026mobileworldmodel}.

This distinction should not be interpreted as claiming that action conditioning automatically 
produces a causal model. When training trajectories come from operational logs, action 
selection can be correlated with traffic conditions, alarms, existing policies, and other 
unobserved factors. Controlled experiments and simulation can provide cleaner interventions, 
while observational action logs require appropriate care. In this article, we therefore use 
the more precise notion of \emph{action-conditioned what-if prediction}: the model estimates 
future network behavior under candidate actions within the support provided by its training 
and calibration data.

\subsection{The Observation--Intervention Asymmetry}
\label{subsec:data_asymmetry}

The challenge is that action-conditioned modeling requires a substantially different data 
regime from ordinary forecasting. Passive telemetry is produced continuously as a by-product 
of network operation. A mobile operator can therefore accumulate months or years of KPI 
measurements, counters, traffic traces, alarms, configuration snapshots, and topology states 
without deliberately changing the network for data collection.

Intervention trajectories are inherently more expensive. An informative trajectory must 
contain not only the network state but also a clearly identified control action and sufficient 
post-action observations to characterize its consequences. In a production network, many 
candidate actions cannot be explored arbitrarily because they may reduce coverage, capacity, 
reliability, or user experience. Moreover, actions that do appear in operational history tend 
to follow existing control policies, resulting in highly non-uniform coverage of the action 
space.

This asymmetry creates an important limitation for a world model trained only from 
action-conditioned trajectories. Such a model ignores potentially much larger volumes of 
action-free observations that contain useful information about traffic dynamics, correlations 
among KPIs, temporal regularities, topology-dependent behavior, and the evolution of network 
states under changing environmental conditions. More importantly, when intervention data are 
scarce, the learned representation itself must be estimated from the same limited dataset that 
is also being used to identify action effects.

A more data-efficient strategy is to separate these two learning problems. General structure 
in network observations can first be learned from the largest available passive dataset. 
Action-conditioned data can then be reserved for the narrower task of learning how control 
decisions modify the already learned network dynamics. This separation is particularly 
attractive for telecom networks because it aligns the training process with the way data are 
actually generated in operational systems.

The principle resembles the separation between large-scale observational pretraining and 
limited interaction-based post-training demonstrated by V-JEPA~2 and its action-conditioned 
variant \cite{assran2025vjepa2}. In that work, an action-free predictive model is first learned 
from large amounts of video and is subsequently adapted into a latent action-conditioned world 
model using substantially less robot interaction data. The data modality and application are 
very different from mobile-network control, but the underlying data-efficiency principle is 
closely aligned with the observation--intervention asymmetry described above.

\subsection{JEPA as an Observation-First Route to Action-Conditioned Dynamics}
\label{subsec:why_jepa_arch}

The remaining question is why JEPA is a suitable mechanism for implementing this staged 
learning strategy. The answer is not that JEPA is the only model family that can benefit from 
pretraining. Time-series Transformers and foundation models can also be pretrained on passive 
network observations and subsequently adapted to downstream tasks. Rather, JEPA offers three 
properties that jointly match the requirements of a control-oriented telecom world model.

First, JEPA learns predictive relationships in representation space. In I-JEPA, a predictor 
estimates representations of target regions from contextual representations rather than 
reconstructing the original image itself \cite{assran2023ijepa}. V-JEPA extends this principle 
to temporal observations and shows that latent feature prediction can capture both appearance 
and motion information from video \cite{bardes2024vjepa}. For telecom data, the analogous goal 
is to learn a compact latent network state that retains information useful for predicting 
network evolution while avoiding the requirement to reconstruct every individual counter, log 
field, or noisy measurement.

Second, representation learning can be performed without action labels. This is essential 
because the majority of available telecom telemetry does not correspond to deliberately 
designed interventions. Predictive pretraining can exploit these observations to learn temporal 
structure, correlations among network variables, and state representations before 
action-conditioned trajectories are introduced.

Third, the predictor can subsequently be extended to incorporate actions while retaining the 
representation learned during observational pretraining. V-JEPA~2-AC provides a concrete 
demonstration of this observation-first, action-later formulation: an action-free JEPA is 
pretrained at large scale, after which an action-conditioned predictor is learned from a much 
smaller interaction dataset \cite{assran2025vjepa2}. Our use of JEPA follows this learning 
principle rather than directly transferring the visual architecture.

Recent wireless research suggests that latent predictive learning is also meaningful for 
communication data. Bou Chaaya \emph{et al.} jointly learn a CSI encoder and a predictive 
latent model to capture wireless channel dynamics \cite{bouchaaya2025latent}. Naoumi 
\emph{et al.} further formulate wireless CSI evolution as an action-conditioned latent world 
model and impose structured transitions on the learned representation 
\cite{naoumi2026structured}. Related work on Time-Series JEPA has also shown that JEPA-style 
representations can support predictive remote control over capacity-limited wireless networks 
\cite{girgis2026tsjepa}. These studies demonstrate the broader applicability of JEPA beyond 
visual data, although their primary targets are channel dynamics, sensing, or remote-control 
representations rather than the controlled evolution of the mobile network itself.

Our formulation therefore occupies a distinct point in this design space. Conventional 
forecasting models primarily learn observational evolution; model-free RL primarily learns a 
policy; direct action-conditioned world models learn network dynamics from intervention 
trajectories; and the proposed action-conditioned JEPA first learns a reusable latent dynamics 
representation from passive telemetry and then specializes that representation using scarce 
action-conditioned data. The resulting hypothesis is experimentally testable: if the staged 
learning principle is well matched to telecom data, its advantage should become increasingly 
visible as the amount of available intervention data decreases.

This observation directly motivates the evaluation methodology adopted later in the article. 
Rather than asking only whether the proposed model achieves lower prediction error under a 
fixed training dataset, we vary the amount of action-conditioned training data and examine how 
passive JEPA pretraining affects future-state prediction, candidate-action evaluation, and 
closed-loop network-control performance. In this way, the evaluation tests the central claim 
of the article---that the primary benefit of action-conditioned JEPA for mobile-network 
control lies in learning useful control-oriented dynamics under severe 
observation--intervention data imbalance.
